Founded World Views with Autoepistemic Equilibrium Logic

Defined by Gelfond in 1991 (G91), epistemic specifications (or programs) are an extension of logic programming under stable models semantics that introducessubjective literals. A subjective literal al-lows checking whether some regular literal is true in all (or in some of) the stable models of the program, being those models collected in a setcalledworld view. One epistemic program may yield several world views but, under the original G91 semantics, some of them resulted from self-supported derivations. During the last eight years, several alternative approaches have been proposed to get rid of these self-supported worldviews. Unfortunately, their success could only be measured by studying their behaviour on a set of common examples in the literature, since no formal property of "self-supportedness" had been defined. To fill this gap, we extend in this paper the idea of unfounded set from standard logic programming to the epistemic case. We define when a world view is founded with respect to some program and propose the foundedness property for any semantics whose world views are always founded. Using counterexamples, we explain that the previous approaches violate foundedness, and proceed to propose a new semantics based on a combination of Moore's Autoepistemic Logic and Pearce's Equilibrium Logic. The main result proves that this new semantics precisely captures the set of founded G91 world views.

==> table.tex <==
\begin{figure}
% [20]{R}{0.33\textwidth}
\small
\begin{tabular}{ | L{1.75cm} | C{2cm}  | }
\hline
program & world views
\\\hline
\multirow{2}{*}{$a \vee b$} &   \multirow{2}{*}{ \sset{\set{a} , \set{b}} }
\\
&
\\\hline
$a \vee b$ &  \multirow{2}{*}{\sset{\set{a} , \set{b}} }
\\
$a \leftarrow \bK b$ &
\\\hline
$a \vee b$ & \multirow{2}{*}{\sset{\set{a} }  }
\\
$a \leftarrow \neg\!\bK b$ & 
% \\\hline
% \end{tabular}
% \hspace{0.2cm}
% \begin{tabular}{ | L{1.75cm} | C{2cm}  | }
% \hline
% program & world views
\\\hline
$a \vee b$ & \multirow{2}{*}{\sset{\set{a,c}, \set{b,c} } }
\\
$c \leftarrow \neg\!\bK b$ & 
\\\hline
$a \leftarrow \neg\!\bK b$ & \multirow{2}{*}{\sset{\set{a}} , \sset{\set{b} } }
\\
$b \leftarrow \neg\!\bK a$ & 
\\\hline
% $a \leftarrow \neg\!\bK b$ &  \multirow{2}{*}{\sset{\set{a}} \,,\, \sset{\set{b} } }
% \\
% $b \leftarrow \neg\!\bK a$ &
% \\\hline
% \end{tabular}
% \hspace{0.2cm}
% \begin{tabular}{ | L{1.75cm} | C{1.7cm}  | }
% \hline
% program & world views
% \\\hline
$a \leftarrow \neg\!\bK\!\neg a$ &  \multirow{2}{*}{\sset{\set{a}}  }
\\
$a \leftarrow \neg\!\bK a$ &
\\\hline\multicolumn{2}{l}{}
\\\multicolumn{2}{l}{}
\\
\end{tabular}
\hspace{1cm}
\begin{tabular}{ | L{2cm} | C{2.6cm} | C{2cm} | }
\hline
program & G91/G11/FAEEL & K15/F15/S17
\\\hline
$a \leftarrow \neg\!\bK\!\neg a$ & 
	 \sset{\emptyset } , \sset{\set{a}} 
	&
	 \sset{\set{a} } 
\\\hline
$a \vee b$ & \multirow{2}{*}{ \text{none} }
&
 \multirow{2}{*}{\sset{\set{a} } } 
\\
$a \leftarrow \neg\!\bK\!\neg b$ & 
 
&
 
\\\hline
$a \vee b$ &  \multirow{2}{*}{ \sset{\set{a}} ,  \sset{\set{a} , \set{b} } }
&
 \multirow{2}{*}{ \sset{\set{a} , \set{b} } } 
\\
$a \leftarrow \bK\!\neg b$ &   
&

\\\hline
$a \leftarrow b$ &
 \multirow{2}{*}{\sset{\emptyset} , \sset{\set{a,b}}  } 
&
 \multirow{2}{*}{\sset{\set{a,b}}  } 
\\
$b \leftarrow \neg\!\bK\!\neg a$ &

&

\\\hline
$a \leftarrow \neg\!\bK\!\neg b$ &  
\multirow{2}{*}{\sset{\emptyset} , \sset{\set{a} , \set{b} } }
&
\multirow{2}{*}{\sset{\set{a} , \set{b} } }
\\
$b \leftarrow \neg\!\bK\!\neg a$ &
&
\\\hline\multicolumn{3}{c}{}
\\\multicolumn{3}{c}{}
\\\multicolumn{3}{c}{}
\\\multicolumn{3}{c}{}
\\\multicolumn{3}{c}{}
\end{tabular}
\vspace{-0.5cm}

\begin{tabular}{ | L{3.9cm} | C{1.95cm} | C{1.95cm} | C{1.95cm} | C{1.95cm} | }
\hline
program & G91 & G11/FAEEL & K15 & F15/S17
\\\hline
$a \leftarrow \neg\!\bK\!\neg b \wedge \neg b$ &  \multicolumn{3}{c|}{\multirow{2}{*}{\sset{\emptyset} , \sset{\set{a} , \set{b} } }}
& \multirow{2}{*}{$\sset{ \set{a}, \set{b} }$}
\\
$b \leftarrow \neg\!\bK\!\neg a \wedge \neg a$ & \multicolumn{3}{c|}{}
&
\\\hline
$a \leftarrow \bK a$ & 
	\sset{\emptyset } , \sset{\set{a}}
	&
	\multicolumn{3}{c|}{ \sset{\emptyset } }
\\\hline
$a \leftarrow \bK a$ & \multirow{2}{*}{ \sset{\set{a}} }
	& \multicolumn{3}{c|}{ \multirow{2}{*}{  \text{none} } }
\\
$a \leftarrow \neg\!\bK a$ & & \multicolumn{3}{c|}{}
\\\hline
\end{tabular}
\caption{The top left table shows a list of examples where G91, G11, K15, F15, S17 and FAEEL agree. The top right table contains examples where FAEEL agrees with G91 and G11 but differs from K15, F15 and S17, which agree among them.
Finally, the bottom table shows a list of examples that further splits these semantics.
Though no example in this list allows to distinguish between G11 and FAEEL, Examples~\ref{ex:unfounded} and~\ref{ex:nog91} in the paper can be used for that purpose.}\label{table:agreement}
\end{figure}

==> table1a.tex <==
\begin{wrapfigure}{r}{0.33\textwidth}
\small
\begin{tabular}{ | C{1.75cm} | C{2cm}  | }
\hline
program & world views
\\\hline
\multirow{2}{*}{$a \vee b$} &   \multirow{2}{*}{ \sset{\set{a} , \set{b}} }
\\
&
\\\hline
$a \vee b$ &  \multirow{2}{*}{\sset{\set{a} , \set{b}} }
\\
$a \leftarrow \bK b$ &
\\\hline
$a \vee b$ & \multirow{2}{*}{\sset{\set{a} }  }
\\
$a \leftarrow \neg\!\bK b$ & 
\\\hline
$a \vee b$ & \multirow{2}{*}{\sset{\set{a,c}, \set{b,c} } }
\\
$c \leftarrow \neg\!\bK b$ & 
\\\hline
$a \leftarrow \neg\!\bK b$ & \multirow{2}{*}{\sset{\set{a}} , \sset{\set{b} } }
\\
$b \leftarrow \neg\!\bK a$ & 
\\\hline
$a \leftarrow \neg\!\bK\!\neg a$ &  \multirow{2}{*}{\sset{\set{a}}  }
\\
$a \leftarrow \neg\!\bK a$ &
\\\hline\multicolumn{2}{l}{}
\\\multicolumn{2}{l}{}
\\
\end{tabular}
\vspace{-0.5cm}

\caption{A list of examples where G91, G11, K15, F15, S17 and FAEEL agree.}\label{table:agreement}
\end{wrapfigure}
